Communication Delay Co-Design in $\mathcal{H}_2$ Distributed Control Using Atomic Norm Minimization

When designing distributed controllers for large-scale systems, the actuation, sensing and communication architectures of the controller can no longer be taken as given. In particular, controllers implemented using dense architectures typically outperform controllers implemented using simpler ones -- however, it is also desirable to minimize the cost of building the architecture used to implement a controller. The recently introduced Regularization for Design (RFD) framework poses the controller architecture/control law co-design problem as one of jointly optimizing the competing metrics of controller architecture cost and closed loop performance, and shows that this task can be accomplished by augmenting the variational solution to an optimal control problem with a suitable atomic norm penalty. Although explicit constructions for atomic norms useful for the design of actuation, sensing and joint actuation/sensing architectures are introduced, no such construction is given for atomic norms used to design communication architectures. This paper describes an atomic norm that can be used to design communication architectures for which the resulting distributed optimal controller is specified by the solution to a convex program. Using this atomic norm we then show that in the context of $\mathcal{H}_2$ distributed optimal control, the communication architecture/control law co-design task can be performed through the use of finite dimensional second order cone programming.

==> algo.tex <==
\subsection{Co-Design Algorithm and Solution Properties}
\label{sec:algo}
In this section we formally define the communication architecture/control law co-design algorithm in terms of the optimization problem \eqref{eq:long_opt}, and show that it can be used to co-design a strongly connected communication graph $\Gamma$ that generates a QI subspace $\s(\Gamma)$ as defined in \eqref{eq:s_gam}. 
%something about how the algorithm consists of two steps: one to get the comm graph, and one to get the controller restricted to it.  We discuss the need for this latter refinement step after an overview of the algorithm.


\begin{algorithm}
 \Input{regularization weight $\lambda$, generalized plant $G$, base QI communication graph $\Gamma_{\text{base}}$, edge set $\mathscr{E}$;}
 \Output{designed communication graph adjacency matrix $\Gamma_{\text{des}}$, optimal Youla parameter $Q^\star_{\text{des}}\in \s(\Gamma_{\text{des}})$; }
 \KwInitialize{$\Gamma_{\text{des}} \leftarrow \Gamma_{\text{base}}$, $Q^\star_{\text{des}} \leftarrow 0$;}
 
 \KwGenGraph{
 $\left(V^\star,\{V^\star_{ij}\},V^\star_{\text{base}}\right) \leftarrow$ solution to optimization problem \eqref{eq:long_opt} with regularization weight $\lambda$;
 
 \ForEach(){$(i,j)\in\mathscr{E}$ s.t. $V^\star_{ij}\neq 0$}{$\Gamma_{\text{des}} \leftarrow \Gamma_{\text{des}} + E_{ij}; $}
}
\KwGetK{
$Q^\star_{\text{des}} \leftarrow$ solution to optimization problem \eqref{eq:quad_prog} with distributed constraint $\Y(\Gamma_{\text{des}})$, as specified by Theorem \ref{thm:quad};
}
\Return{$\Gamma_{\text{des}}$, $Q^\star_{\text{des}}$;}
 \caption{Communication Architecture Co-Design}
 \label{lag:co-design}
\end{algorithm}
%logical flow
%solve reg opt to get structure, then solve quad opt to get optimal controller... by varying lambda, we go from base graph (very large lambda) and corresponding minimal optimal controller Kbase and closed loop performance nubase to maximal graph (0 lambda) and corresponding minimal optimal controller Kbase and closed loop performance nubase,  
%we prove that the structure of C(V) defines a graph Gam in G, and hence S(Gam) is QI

The co-design procedure is described in Algorithm \ref{lag:co-design}.  The algorithm consists of first solving the regularized optimization problem \eqref{eq:long_opt} to obtain solutions $\left(V^\star,\{V^\star_{ij}\},V^\star_{\text{base}}\right)$.  Using these solutions, we produce the designed communication graph $\Gamma_{\text{des}}$ by augmenting the base QI communication graph $\Gamma_{\text{base}}$ with all edges $(i,j)$ such that $V^\star_{ij} \neq 0$.  In particular, each non-zero term $V^\star_{ij}$ corresponds to an additional edge $(i,j) \in \mathscr{E}$ that the co-designed distributed control law will use -- thus by varying the regularization weight $\lambda$ the controller designer can control how much the use of an additional link is penalized by the optimization problem \eqref{eq:long_opt}.  As $\supp{\Gamma_{\text{base}}}\subseteq\supp{\Gamma_{\text{des}}}\subseteq\supp{\Gamma_{\text{max}}}$ by construction, the designed communication graph $\Gamma_{\text{des}}$ satisfies the assumptions of Proposition \ref{prop:space} -- it is therefore strongly connected, can be physically built, and generates a subspace $\s(\Gamma_{\text{des}})$, according to \eqref{eq:s_gam}, that is QI with respect to $G_{22}$ and that admits a decomposition of the form \eqref{eq:s_decomp}.  
The subspace $\s(\Gamma_{\text{des}})$ thus satisfies the assumptions of Theorem \ref{thm:quad}, meaning that the distributed optimal controller $K^\star_{\text{des}}$ restricted to the designed subspace $\s({\Gamma_{\text{des}}})$ is specified in terms of the solution $Q^\star_{\text{des}}$ to the convex quadratic program \eqref{eq:quad_prog}.  In this way the optimal distributed controller restricted to the designed communication architecture, as well as the performance that it achieves, can be computed exactly.

\edit{Although the solution $V^\star$ to optimization problem \eqref{eq:long_opt} could be used to generate a distributed controller that can be implemented on the designed communication graph $\Gamma_{\text{des}}$, we claim that it is preferable to use the solution $Q^\star_{\text{des}}$ to the non-regularized optimization problem \eqref{eq:quad_prog}.  First, the use of a regularizer in a linear inverse problem (of which \eqref{eq:quad_prog} is a special case) has the effect of shrinking its solution towards the origin.  In our case, this means that the resulting controller specified by $V^\star$ is less aggressive, i.e., has smaller control gains, than the controller specified by the solution to the optimization \eqref{eq:quad_prog} with subspace constraint $\Y(\Gamma_{\text{des}})$.}

Second, notice that for two graphs $\Gamma_{ij}$ and $\Gamma_{kl}$ obtained by augmenting the base QI communication graph $\Gamma_{\text{base}}$ with the communication links $(i,j)$ and $(k,l)$, respectively, it holds that $\s(\Gamma_{ij}) + \s(\Gamma_{kl}) \subseteq \s(\supp{\Gamma_{ij} +\Gamma_{kl}})$, with the inclusion being strict in general.
In words, the linear superposition of the subspaces \eqref{eq:s_gam} generated by the two communications graphs $\Gamma_{ij}$ and $\Gamma_{kl}$ is in general a strict subset of the subspace generated by the single communication graph $\supp{\Gamma_{ij}+\Gamma_{kl}}$.  Suppose now that the corresponding solutions $V_{ij}^\star$ and $V^\star_{kl}$ to optimization problem \eqref{eq:long_opt} are non-zero: then $\Gamma_{\text{des}}=\Gamma_{\text{base}} + E_{ij} + E_{kl}$, but the expression $\mathfrak{C}(V^\star)$ lies in the subspace given by $\s(\Gamma_{ij}) + \s(\Gamma_{kl})$.
By the previous discussion $\s(\Gamma_{ij}) + \s(\Gamma_{kl})\subset\s(\Gamma_{\text{des}})$, and thus we are imposing additional structure on the the expression $\mathfrak{C}(V^\star)$ relative to that imposed on the solution to the non-regularized optimization problem \eqref{eq:quad_prog} with subspace constraint $\Y(\Gamma_{\text{des}})$.  This can be interpreted as the controller specified by the structure of $\mathfrak{C}(V^\star)$ not utilizing paths in the communication graph that contain both links $(i,j)$ and $(k,l)$.  These sources of conservatism in the control law are however completely removed if one uses the solution $Q^\star_{\text{des}}$ to the non-regularized optimization problem \eqref{eq:quad_prog}. 

 Thus we have met our objective of developing a convex optimization based procedure for co-designing a distributed optimal controller and the communication architecture upon which it is implemented.  In the next section we discuss the computational complexity of the proposed method and illustrate its efficacy on numerical examples.



%The additional structure imposed on $\mathfrak{C}(V^\star)$ also causes the regularized optimization problem \eqref{eq:long_opt} to under-estimate the benefit of combinations of communication links, which in turn may lead to co-designed communication graphs with a larger number of additional communication links than necessary.  In order to alleviate this, the controller designer may wish to allow the atomic 


%logical flow -- justify refinement step as opposed to using V^* to synthesize an optimal controller.  Two sources of conservatism: 
%NEED TO FIGURE OUT HOW TO INCLUDE THE FACT THAT WE WANT TO INCLUDE AS MANY "EXTRA LINKS" AS POSSIBLE IN THE ATOMIC SET. 
%1)  The addition of a regularizer to the objective of a linear inverse problem (of which \eqref{eq:quad_prog} is a special case) has the effect of shrinking its solution towards the origin.  In our case, this means that the resulting controller specified by $V^*$ is less aggressive, i.e., has smaller control gains, than the controller specified by the solution to the optimization \eqref{eq;quad_prog} with subspace constraint $\Y(\Gamma_{des})$. 
%2) Generically, \supp((G1 + G2)^t)\superset \supp(G1^t + G2^t) -- this is a reflection of the fact that V^* is really a superposition of controllers implemented on their respective graphs, as opposed to a controller implemented on the graph G1 + G2.  In particular the controller resulting from V^* does not route information according to shortest paths on G1+G2 (footnote about how this means that the structure of C(V^*) generally does not correspond to QI subspace) -- however, by solving the optimization problem \eqref{eq:quad_prog} constrained to the subspace $\Y(\Gamma_{des})$, these issues are alleviated.
%toy example to illustrate these issues, and then say that we come back to it with 6 player chain example in next section









==> comm_norm.tex <==
\subsection{The Communication Link Norm}
\label{sec:comm_norm}
Recall that our approach to the co-design task is to induce suitable structure in the expression $\mathfrak{C}\left(V^\star\right)$, where $V^\star$ is the solution to the regularized convex optimization problem \eqref{eq:reg_opt} employing the yet to be specified convex penalty function $\commnorm{\cdot}$.  We argued that the structure induced in the expression $\mathfrak{C}\left(V^\star\right)$ should correspond to strongly connected communication graphs that generate QI subspaces of the form \eqref{eq:s_decomp}, as this allows us to leverage Theorem \ref{thm:quad} to solve for the distributed optimal controller restricted to such a subspace. We then characterized the QI communication graph design set $\mathscr{G}$ -- which is composed of communication graphs that generate subspaces \eqref{eq:s_gam} that are QI with respect to a plant $G_{22}$ --  in terms of a base QI communication graph $\Gamma_{\text{base}}$ and a maximal QI communication graph $\Gamma_{\max}$.

To explore the QI communication graph design set $\mathscr{G}$, we begin with the base QI communication graph $\Gamma_{\text{base}}$ and augment it with additional communication links drawn from the set $\mathscr{E}$.  The convex penalty function $\commnorm{\cdot}$ used in the regularized optimization problem \eqref{eq:reg_opt} should therefore penalize the use of such additional communication links -- in this way the controller designer can tradeoff between communication complexity and closed loop performance by varying
the regularization weight $\lambda$ in optimization problem \eqref{eq:reg_opt}.

It is conceptually useful to view a distributed controller implemented using a dense communication graph as being composed of a superposition of simple \emph{atomic} controllers that are implemented using simple communication graphs, i.e., using communication graphs that can be obtained by adding a small number of edges to the base QI communication graph.  This viewpoint suggests choosing the convex penalty function $\commnorm{\cdot}$ to be an atomic norm \approxcitations, \cite{CRPW12}.

Indeed, if one seeks a solution $X^\star$ that can be composed as a linear combination of a small number of atoms drawn from a set $\A$, then a useful approach, as described in  \cite{CRPW12,CDS98,CRT06,Donoho04, fazelThesis,RFP10,CR12}, to induce such structure in the solution of an optimization problem is to employ a convex penalty function that is given by the atomic norm induced by the atoms $\A$ \cite{Bon91,Pis86}. Examples of the types of structured solutions one may desire include sparse, group sparse and signed vectors,  and low-rank, permutation and orthogonal matrices \cite{CRPW12}.

Specifically, if one desires a solution $X^\star$ 
that admits a decomposition of the form
\begin{equation}
X^\star=\sum_{i=1}^{r}c_{i}A_{i},\ A_{i}\in\A,\ c_{i}\geq0
\label{eq:decomp}
\end{equation}
for a set of appropriately scaled and centered atoms $\A$,
and a small number $r$ relative to the ambient dimension, then solving
\begin{equation}
\begin{array}{rl}
\underset{X}{\mathrm{minimize}}  &  \Htwonorm{\mathfrak{A}(X)}^2 + \lambda\|X\|_\A
\end{array}
\end{equation}
with $\mathfrak{A}(\cdot)$ an affine map, and the atomic norm $\|\cdot\|_\A$ given by the gauge function\footnote{If no {such $\theta$ exists}, then $\|X\|_\A = \infty$.} 
\begin{equation}
\begin{array}{rcl}
\|X\|_{\A}: & = & \inf\left\{\theta\geq0\, \big{|}\, X\in \theta\mathrm{conv}(\A)\right\}\\
 & = & \inf\left\{\sum_{A\in\A}c_{A}\, \big{|}\, X=\sum_{A\in\A}c_{A}A,\, c_A \geq 0\right\}
\end{array}
\label{eq:atom_norm}
\end{equation}
results in solutions that are both consistent with the data as measured in terms of the cost function $\Htwonorm{\mathfrak{A}(X)}^2$, and that \edit{ admit sparse atomic decompositions, i.e., that are a combination of a small number of elements from $\A$. }

We can therefore fully characterize our desired convex penalty function $\commnorm{\cdot}$ by specifying its defining atomic set $\A_{\text{comm}}$ and then invoking definition \eqref{eq:atom_norm}.  As alluded to earlier, we choose the atoms in $\A_{\text{comm}}$ to correspond to distributed controllers implemented on communication graphs that can be constructed by adding a small number of communication links from the set of allowed edges $\mathscr{E}$ to the base QI communication graph $\Gamma_{\text{base}}$.  In order to avoid introducing additional notation we describe the atomic set specified by communication graphs that can be constructed by adding a single communication link from the set $\mathscr{E}$ to the base QI communication graph $\Gamma_{\text{base}}$ -- the presented concepts then extend to the general case in a natural way.  We explain why a controller designer may wish to construct an atomic set specified by more complex communication graphs in \S\ref{sec:discussion}.

\subsubsection*{The atomic set  $\A_{\text{comm}}$}To each communication link $(i,j) \in \mathscr{E}$  we associate the subspace $\mathcal{E}_{ij}$ given by
\begin{equation}
\mathcal{E}_{ij} := \s^\perp(\Gamma_{\text{base}})\cap \s(\Gamma_{\text{base}} + E_{ij}).
\label{eq:link_space}
\end{equation}
In words, the subspace $\mathcal{E}_{ij}$ corresponds to the additional information available to the controller relative to the base communication graph $\Gamma_{\text{base}}$ uniquely due to the added communication link $(i,j)$ from sub-controller $j$ to sub-controller $i$.  Note that the subspaces $\mathcal{E}_{ij}$ are finite dimensional due to the strong connectedness assumption imposed on $\Gamma_{\text{base}}$, which leads to the equality $\s^\perp(\Gamma_{\text{base}}) = \Y^\perp(\Gamma_{\text{base}})\cap\RHinf^{\leq d(\Gamma_{\text{base}})}$.
\begin{example}
Consider the base QI communication graph $\Gamma_{\text{base}}$ illustrated in Figure \ref{fig:4chain} and specified by \eqref{eq:3-chain_gam}.  This communication graph generates the subspace $\s(\Gamma_{\text{base}})$ shown in \eqref{eq:3-chain_s}.
We consider choosing from two additional links to augment the base communication graph $\Gamma_{\text{base}}$: a directed link from node 1 to node 3, and a directed link from node 3 to node 1.  Then $\mathscr{E} = \{(1,3),(3,1)\}$ and the corresponding subspaces $\mathcal{E}_{ij}$ are given by
\begin{equation*}
\begin{array}{rclrcl}
\mathcal{E}_{13} &=& \frac{1}{z^2}\begin{bmatrix} 0 & 0 & 0  \\  0 & 0 & 0 \\ \ast & 0 & 0 \end{bmatrix}, 
\mathcal{E}_{31} &=& \frac{1}{z^2}\begin{bmatrix} 0 & 0 & \ast  \\  0 & 0 & 0 \\ 0 & 0 & 0 \end{bmatrix}.
\end{array}
\end{equation*}
\hfill{}\QED
\end{example}

The atomic set is then composed of suitably normalized elements of these subspaces:
\begin{equation}
\edit{\A_{\text{comm}}:= \displaystyle\bigcup_{(i,j) \in \mathscr{E}}\left\{ V \in \mathcal{E}_{ij} \, \big{|} \, \Htwonorm{V} = 1 \right\}.}
\label{eq:comm_set}
\end{equation}
Note that we normalize our atoms relative to the $\Htwo$ norm as this norm is isotropic; hence this normalization ensures that no atom is preferred over another within the family of atoms defined by a subspace $\mathcal{E}_{ij}$.
The resulting atomic norm,\footnote{\edit{We apply definition \eqref{eq:atom_norm} to the components of $X$ that lie in $\s^\perp(\Gamma_{\text{base}})$ to obtain an atomic norm defined on elements of that space.  We then introduce an unpenalized variable $V_\text{base}\in \Y(\Gamma_{\text{base}})$ to the atomic decomposition so that the resulting penalty function may be applied to elements $X \in \RHinf^{\leq d(\Gamma_\text{base})}$.  The resulting penalty is actually a seminorm on $\RHinf^{\leq d(\Gamma_\text{base})}$ but we refer to it as a norm to maintain consistency with the terminology of \cite{CRPW12}.}} which we denote the \emph{communication link norm}, is given by \edit{
\begin{equation}
\begin{array}{rl}
\commnorm{X} = \edit{\minimize{V_{\text{base}},\left\{V_{ij}\right\}\in\RHinf^{\leq d(\Gamma_\text{base})}}} & \sum_{(i,j)\in\mathscr{E}}\Htwonorm{V_{ij}} \\
\text{s.t.} & X = V_{\text{base}} + \sum_{(i,j) \in \mathscr{E}}V_{ij} \\
&V_{\text{base}} \in \Y(\Gamma_{\text{base}}) \\
& V_{ij} \in \mathcal{E}_{ij} \ \forall (i,j) \in \mathscr{E},
\end{array}
\label{eq:comm_norm}
\end{equation}
when this optimization problem is feasible --  when it is not, we set $\commnorm{X} = \infty$.  An element $V_{ij}\in\E_{ij}$ of the atomic decomposition of an element $X$ is nonzero in optimization problem \eqref{eq:comm_norm} if a link from sub-controller $j$ to sub-controller $i$ must be present in...  Given this correspondence between nonzero $V_{ij}$ and the use of communication link $(i,j)$, and the form of the optimization problem also makes it clear that solutions with sparse communication link usage are promoted. \todo{this is shit, fix it}  }

Using this penalty function in the regularized optimization problem \eqref{eq:reg_opt} yields the convex optimization problem
\begin{equation}
\begin{array}{rl}
 \edit{\minimize{V,V_{\text{base}},\left\{V_{ij}\right\}\in\RHinf^{\leq d(\Gamma_\text{base})}}} & \Htwonorm{\mathfrak{L}(V)}^2 + \lambda \left(\sum_{(i,j)\in\mathscr{E}}\Htwonorm{V_{ij}} \right)\\
\text{s.t.} & \mathfrak{C}(V) = V_{\text{base}} + \sum_{(i,j) \in \mathscr{E}} V_{ij}\\
& V_{\text{base}} \in \Y(\Gamma_{\text{base}}) \\
& V_{ij} \in \mathcal{E}_{ij} \ \text{for all }(i,j) \in \mathscr{E}.
\end{array}
\label{eq:long_opt}
\end{equation}
Let  $\left(V^\star,\{V^\star_{ij}\},V^\star_{\text{base}}\right)$ denote the solution to the optimization problem \eqref{eq:long_opt}. The structure of $\mathfrak{C}(V^\star)$, and consequently the designed communication graph, is then specified by that of $V^\star_{\text{base}}$ and that of the non-zero $\{V^\star_{ij}\}$.  Note further that $V^\star_{\text{base}}$ is not penalized by the communication link norm, and therefore the communication graph defined by the structure of $\mathfrak{C}(V^\star)$ has $\Gamma_{\text{base}}$ as a subgraph.  In what follows, we explain precisely how the structure of $\mathfrak{C}(V^\star)$ can be used to specify a communication graph.

\begin{rem}
Optimization problem \eqref{eq:long_opt} is finite dimensional, and hence can be formulated as a second order cone program by associating the finite impulse response transfer matrices $(V,V_{\text{base}},\left\{V_{ij}\right\})$, $ \mathfrak{C}(V)$ and $\mathfrak{L}(V)$ with their matrix representations.  To see this, note that $\Y(\Gamma_{\text{base}})\subseteq\RHinf^{\leq d(\Gamma_{\text{base}})}$, and that by the discussion after the definition \eqref{eq:link_space} of the subspaces $\mathcal{E}_{ij}$, they too satisfy $\mathcal{E}_{ij}\subseteq\RHinf^{\leq d(\Gamma_{\text{base}})}$. Thus the horizon  $d(\Gamma_{\text{base}})$ over which the optimization problem \eqref{eq:long_opt} is solved is finite.
\label{rem:fin_dim}
\end{rem}

==> discussion.tex <==
\noindent\textbf{Optimal structural recovery:} It is shown in \cite{MC_RFD_TAC} that the variational solution to an $\Htwo$ optimal control problem augmented with an atomic norm that penalizes the use of actuators can succeed in identifying an optimal actuation architecture when the dynamics of the plant satisfy certain conditions.  The numerical experiments of \S\ref{sec:examples} provide empirical evidence that our approach to communication architecture design identifies optimally structured controllers as well -- it is of interest to see whether conditions analogous to those of \cite{MC_RFD_TAC} can provide theoretical support to the empirical success of our approach.  

\noindent\textbf{The $k$-communication link norm:} The communication link norm was defined in terms of atoms corresponding to communication graphs constructed by adding a single link to the base QI communication graph.  However it is possible to include atoms corresponding to communication graphs augmented with at most $k$-links instead, for any positive integer $k$; denote the resulting $k$-communication link norm by $\kcommnorm{k}{\cdot}$.  If the atoms are suitably normalized,\footnote{In particular, elements in $V \in \mathscr{A}_{\text{k-comm}}$ constrained to lie in a subspace $\mathcal{E}$ should be normalized as $\Htwonorm{V} = \left(\text{card}\left(\mathcal{E}\right) + \kappa\right)^{-\frac{1}{2}}$, where $\kappa>0$ is a positive constant that controls how much a single atom of larger cardinality is preferred over several atoms of lower cardinality.} for all positive integers  $k_1$ and $k_2$ satisfying $k_1\leq k_2$
it then holds that $\kcommnorm{k_1}{G} \leq \kcommnorm{k_2}{G}$ for all transfer matrices $G$ satisfying $\kcommnorm{k_1}{G}<\infty$.  Geometrically, restricted to the domain of $\kcommnorm{k_1}{\cdot}$, the unit ball of $\kcommnorm{k_2}{\cdot}$ is an inner approximation to that of $\kcommnorm{k_1}{\cdot}$, and may therefore lead to simpler communication graphs when used as a penalty function in the regularized optimization problem \eqref{eq:reg_opt}.  How to choose $k$ will presumably be informed by the aforementioned conditions on optimal communication structure recovery, as well as by computational considerations, as the number of elements $\{V_{ij}\}$ required to implement the $k$-communciation link norm scales as $O(n^{2k})$.

\noindent\textbf{Constructing base QI communication graphs:}  The assumption of block-diagonal state-space matrices $B_2$ and $C_2$ is necessary to guarantee that the base QI communication graph as specified in \eqref{eq:gam_min} indeed generates a QI subspace.  Likewise the assumption that $\bsupp{A}$ specifies a strongly connected adjacency matrix is necessary to guarantee that the resulting subspace admits a decomposition of the form \eqref{eq:s_decomp}. Exploring how to construct base QI communication graphs in a principled way when the structural assumptions on $(A,B_2,C_2)$ are relaxed, perhaps utilizing the methods in \cite{RM12}, is an interesting direction for future work.  We note however that the rest of the discussion in \S\ref{sec:delays} remains valid once a base QI communication graph is identified even if the structural assumptions on $(A,B_2,C_2)$ are relaxed .  We also note that these issues are a consequence of the communication protocol imposed between sub-controllers -- determining alternative communication protocols that allow the structural assumptions to be relaxed is also an interesting direction for future work.  

\noindent\textbf{Scalability:} Although we expect the methods presented to be applicable to systems composed of hundreds of sub-controllers, it is important that the general approach of the RFD framework be applicable to truly large scale systems composed of heterogeneous sub-systems.  We note that the limits on the scalability of our proposed method are due to the underlying controller synthesis method \cite{LD14}, as opposed to being inherent to the communication link norm.  To that end we have been pursuing \emph{localized optimal control} \cite{WMD_CDC14} as a scalable distributed optimal controller synthesis method -- an interesting direction for future work will be to see if communication architecture co-design can be incorporated into the localized optimal control framework.
%\noindent\textbf{Different performance metrics:} The communication link norm can also be used to augment the variational solutions to distributed control problems with alternative performance metrics.  For example, in \cite{M_CDC14_dhinf} we show that the distributed control problem with an $\Hinf$ performance metric analogous to that considered here can be reduced to a finite dimensional semidefinite program -- augmenting this semidefinite program with the communication link norm would then allow the controller designer to tradeoff between communication complexity and the $\Hinf$ closed loop performance of a distributed controller.
%
%\noindent\textbf{Specialized solvers:} The structure of the regularized optimization problem \eqref{eq:reg_opt} is especially suited to optimization algorithms that allow for the problem to be decomposed, such as the alternating direction method of multipliers (ADMM) \cite{Boyd_ADMM}.  ADMM based approaches have been very successful in the co-design of structured static feedback gains \cite{LFJ13}, and we are optimistic that a specialized solver based on such a method will allow our co-design procedure to scale to problems with 100s of sub-controllers.



==> introduction.tex <==
Large-scale systems represent an important class of application areas for the control engineer -- prominent examples include the smart-grid, software defined networking (SDN) and automated highways.  For such large-scale systems, designing the controller \emph{architecture} -- placing sensors and actuators as well as the communication links between them -- is arguably as important as the traditional design of the control laws themselves.  In this paper we assume that a sensing and actuation architecture is already in place, and focus on designing the communication architecture of a distributed controller that minimizes the $\Htwo$ norm of the closed loop system.\footnote{The Regularization for Design (RFD) framework, introduced in \cite{MC_RFD_TAC}, allows for the simultaneous design of actuation, sensing and communication architectures.  The communication architecture design component of the RFD framework uses the methods developed in this paper.}

In particular, a distributed controller can be viewed as a collection of sub-controllers, each equipped with a set of actuators and sensors, that exchange their respective measurements with each other subject to \emph{communication delays} imposed by an underlying communication graph.  
We view dense communication architectures (i.e., ones with a large number of communication links between sub-controllers) as being composed of multiple simple \emph{atomic} communication architectures (i.e., ones with a small number of communication links between sub-controllers).  Although in general controllers with dense communication schemes will outperform controllers with sparser ones, it is desirable to minimize the cost of building the communication architecture needed to implement the controller.  Thus the problem of controller communication architecture/control law co-design can be framed as the joint optimization of a suitably defined measure of the communication complexity of the distributed controller and its closed loop performance, in which these two competing metrics are traded off against each other in a principled manner.

The question that then needs to be addressed is what properties should the designed communication architecture satisfy?  In general one can select communication architectures that range in complexity from completely decentralized (i.e., distributed controllers with no communication allowed between sub-controllers) to essentially centralized and without delay (i.e., distributed controllers with instantaneous communication allowed between all sub-controllers).  However, if we demand that the distributed optimal controller restricted to the designed communication architecture be specified as the solution to a finite dimensional convex optimization problem, this limits the simplicity of the desired communication architecture \cite{W68}\cite{RL06},\cite{RCL10},\cite{LL11}.  In particular a sufficient, and under mild assumptions necessary, condition for a distributed optimal controller to be specified by the solution to a convex optimization problem\footnote{For a more detailed overview of the relationship between information exchange constraints and the convexity of distributed optimal control problems, we refer the reader to \cite{RL06,RCL10,MMRY12} and the references therein.}  is that the communication architecture allow sub-controllers to communicate with each other as quickly as their control actions propagate through the plant \cite{RCL10}.  Although this condition may seem restrictive, it can often be met in practice by constructing a communication topology that mimics or is a superset of the physical topology of the plant.  For example, these delay based conditions could be satisfied in a smart-grid setting by laying down fiber-optic cables in parallel to transmission lines; in a SDN setting by giving control packets priority in routing protocols; and in an automated highway system setting by allowing vehicles to communicate wirelessly with nearby vehicles.

%Since this paper is about communication architecture design, I can ask the question of what type of architecture do we want to design and why?  I?d want something QI because it leads to convex optimal control problems, and I?d want something strongly connected because it makes these convex problems finite dimensional.  A simple condition for QI to hold is that the comms match the plant, something that can be generally accomplished in practice, e.g. in the power grid we would lay fiber optic cables along the power lines, in SDN we would give priority to control packets and in automated highway systems comms is wireless by the dynamics are decoupled.


%A useful approach to modeling a distributed plant is to view it as a collection of subplants that interact with each other according to \emph{propagation delays} imposed by their physical interconnection.  Likewise, a distributed controller can be viewed as a collection of sub-controllers, each equipped with a set of actuators and sensors, that exchange their respective measurements with each other subject to \emph{communication delays} imposed by an underlying communication graph.  
%With this view of distributed systems and distributed controllers, the communication architecture/control law co-design task is then to find a minimal set of communication links between sub-controllers such that a desired closed loop performance is achieved.  
%We additionally impose that the distributed optimal controller restricted to the designed communication architecture be linear and be specified by the solution to a convex optimization problem.  When these conditions on hold, it is then possible to determine the optimal performance achievable by a distributed controller implemented using the designed communication architecture, along with the optimal control law itself, allowing for a meaningful assessment of the quality of said architecture.

When the aforementioned delay based condition is satisfied by a distributed constraint, it is said to 
% In \cite{RL06}, the broadest known characterization of such convex distributed optimal control problems was made in terms of 
be \emph{quadratically invariant} (QI) \cite{RL06}.  Although quadratic invariance guarantees convexity of the resulting distributed optimal control problem, it may still be infinite dimensional.  Recently it has been shown that in the case of $\Htwo$ distributed optimal control subject to QI constraints imposed by a strongly connected communication architecture, i.e. one in which every sub-controller can exchange information with every other sub-controller subject to delay, the resulting distributed optimal controller synthesis problem can be reduced to a finite dimensional convex program that admits an efficient solution \cite{LDXX,LD14}.\footnote{Other solutions exist to the $\Htwo$ distributed control problem subject to delay constraints -- we refer the reader to the discussion and references in \cite{LD14} for a more extensive overview of this literature.}  In light of these observations, we therefore look to design \emph{strongly connected communication architectures} that induce \emph{QI} constraint sets -- once such a communication architecture is obtained, the methods from \cite{LDXX,LD14} can then be used to compute the optimal distributed controller restricted to that communication architecture exactly.

%
%
%Although we build on the methods presented in \cite{LDXX,LD14} to solve the $\Htwo$ distributed control problem subject to delays (which we review in \S \ref{sec:H2mm}),  we note that alternative solutions exist to this and other closely related controller synthesis problems, and refer the reader to \cite{LD14} for an extensive review of this literature.
%
%
%To solve the communication architecture/control law co-design problem, we observe that specific sparsity patterns in the impulse response elements of the controller have a direct interpretation in terms of the communication graph used by the controller, and hence we seek suitably structured solutions to the underlying distributed optimal controller synthesis problem.
To that end, we show that the communication complexity of a distributed controller can be inferred from the structure of its impulse response elements, allowing us to formulate the communication architecture/control law co-design task as one of seeking suitably structured solutions to an underlying controller synthesis problem.  
Inducing suitable structure in the solution to an optimization problem is of interest in a broad range of applications in applied mathematics, e.g., computing sparse solutions to linear inverse problems or computing low-rank solutions to systems of linear matrix equations is a problem that arises in signal processing and in statistics \ellcitations, \nuccitations. These ideas were extended in \cite{CRPW12}, where the authors describe a generic convex programming approach -- based on minimizing an appropriate \emph{atomic norm} \approxcitations$\text{ }$  -- for inducing a desired type of structure in solutions to linear inverse problems.  

Motivated by these developments, our approach to the problem of joint communication architecture/control law co-design is to augment the variational formulation of the solution to the $\Htwo$ distributed optimal controller synthesis problem presented in \cite{LD14} with a suitable convex regularization function.% such that the structure of the solution to the regularized optimization problem corresponds to a strongly connected communication graph that induces a quadratically invariant constraint set.

%
%By carefully constructing this regularization function, we  ensure that  
%
%Our objective in this paper is to formulate this joint optimization in the context of $\Htwo$ distributed optimal control as a finite dimensional convex optimization problem.  We also ask that the optimal controller restricted to the designed communication architecture be linear and specified by the solution to a convex optimization problem that can be solved exactly.  In \cite{LDXX,LD14}, it is shown that if a strongly connected communication graph induces a \emph{quadratically invariant} \cite{RL06,RCL10} constraint set with respect to the distributed plant, then solving for the corresponding $\Htwo$ distributed optimal controller can be reduced to solving a finite dimensional convex quadratic program subject to affine constraints.  Further, it is seen that these affine constraints encode the communication architecture of the distributed controller.  Building on the results in \cite{LDXX,LD14}, our approach is to remove the affine constraints that encode the communication architecture of the distributed controller from the convex optimization problem, and instead augment the objective of this optimization problem with the a term that penalizes the communication complexity of the controller.




%Our approach is to augment the $\Htwo$ distributed optimal control problem with a suitable penalty such that the solution to the optimization problem specifies a communication architecture that is strongly connected and that induces induce a \emph{quadratically invariant} \cite{RL06,RCL10} constraint set with respect to the given distributed system.  These two properties of the designed communication architecture, namely quadratic invariance and strong connectedness, allow us to leverage the results of \cite{LDXX,LD14} 
%
%The quadratically invariant property of the constraint set ensures that the optimal controller restricted to the designed communication architecture is linear and specified as the solution of a convex optimization problem \cite{RL06,RCL10}.  The strong connectedness of the communication architecture allows us to leverage the recent results in \cite{LDXX,LD14} that reduce the controller synthesis problem to a finite dimensional convex quadratic program.


%The set of possible communication topologies between sub-controllers is combinatorial in cardinality, ranging from completely decentralized (i.e., no communication between sub-controllers) on one extreme to completely centralized (i.e., instantaneous communication between all sub-controllers) on the other.  However it is often the case that instantaneous communication between all sub-controllers is not possible due to finite communication speed and potentially physically dispersed systems.  On the other hand, it is well known that completely decentralized

\textbf{Related Work:}  Regularization techniques based on $\ell_1$ norms and, more generally, atomic norms have already been employed extensively in system identification, e.g., to identify systems of small Hankel order (cf. \cite{SBTR12,Fazel,MR_CDC14}), and in linear regression based methods \cite{LjungNewOld}.  
%Although the resulting solutions yield structured systems, they typically do not have a direct interpretation in terms of the architecture of a control system (i.e., actuators, sensors and the communication links between them).  
The use of regularization explicitly for the purpose of designing the architecture of a controller can also be found in the literature.  Examples include the use of $\ell_1$ regularization to design sparse structures in $\mathcal{H}_2$ feedback gains \cite{LFJ13}, treatment therapies \cite{JRM14}, consensus \cite{DLFM12,XB07} and synchronization \cite{FLJ13} topologies; and the use of group norm penalties to design actuation/sensing schemes \cite{MC_CDC14,DJL14}.  More generally, the Regularization for Design framework \cite{MC_RFD_TAC} builds on the results in this paper and allows for the simultaneous design of the actuation, sensing and communication architectures of a controller.


\textbf{Contributions:}
%We formulate the communication architecture/control law co-design task as one of jointly optimizing the closed loop performance of a distributed controller and the complexity of the communication graph used to implement it, and show that this task can be accomplished via convex programming.  In particular 
We leverage results from distributed optimal control theory \cite{LDXX,LD14} and structured linear inverse problems \cite{CRPW12} to formulate the co-design task as a finite dimensional second order cone program. We propose using a carefully constructed atomic norm  \cite{CRPW12}, \approxcitations, which we call the communication link norm, as a convex penalty function -- intuitively, this norm penalizes the number of additional communication links used by the resulting distributed optimal controller.  We show that augmenting the variational solution to the $\Htwo$ distributed control problem presented in \cite{LDXX,LD14} with the communication link norm as a regularizer induces suitable structure in the solution of the resulting optimization problem.  In particular, the structure of this solution can be used to specify a strongly connected communication graph that leads to QI constraints,
%that is both strongly connected and that leads to quadratically invariant constraints on the distributed controller.  These two properties allow for
allowing for the resulting distributed optimal controller to be specified by the solution to a finite dimensional quadratic program \cite{LD14}. We use these results to formulate a communication architecture/control law co-design algorithm that yields a distributed optimal controller and the communication architecture on which it is to be implemented. By varying the weight on the communication link norm penalty function, the controller designer can use our co-design algorithm to explore the tradeoff between communication architecture complexity and closed loop performance in a principled way via convex optimization.


\textbf{Paper Organization:}
In \S \ref{sec:prelims} we introduce necessary operator theoretic concepts and establish notation.   In \S \ref{sec:problem} we formulate the communication architecture/control law co-design problem as the joint optimization of a suitably defined measure of the communication complexity of a distributed controller and the closed loop performance that this controller achieves.  In \S \ref{sec:delays}, we show how communication graphs can be used to generate distributed constraints, and show that if a communication graph that generates a QI subspace is augmented with additional communication links, the subspace generated by the resulting communication graph is also QI.  We use this observation and techniques from structured linear inverse problems \cite{CRPW12} in \S \ref{sec:co_design} to construct a convex penalty function that penalizes the use of additional communication links by a distributed controller, and formulate the co-design procedure.  We discuss the computational complexity of the co-design procedure in \S \ref{sec:examples} and illustrate the usefulness of our approach with two numerical examples.  We end with a discussion in \S \ref{sec:discussion}.

==> introduction_rfd.tex <==
Large-scale systems represent an important class of application areas for the control engineer -- prominent examples include the smart-grid, software defined networking (SDN) and automated highways.  For such large-scale systems, designing the controller \emph{architecture} -- placing sensors and actuators as well as the communication links between them -- is now also an important part of the controller synthesis process. Indeed controllers with denser actuation, sensing and communication architectures will typically outperform those with simpler architectures -- however economic considerations also dictate that it is desirable to minimize the cost of constructing a controller architecture.
In \cite{MC_RFD_TAC}, the author of this paper and V. Chandrasekaran address the problem of jointly optimizing the architectural complexity of a distributed optimal controller and the closed loop performance that it achieves by introducing the Regularization for Design (RFD) framework.  In RFD, controllers with complicated architectures are viewed as being composed of atomic controllers with simpler architectures -- this family of simple controllers is then used to construct various \emph{atomic norms} \cite{CRPW12}, \approxcitations$\text{ }$ that penalize the use of specific architectural resources, such as actuators, sensors or additional communication links.  These atomic norms are then added as a penalty function to the variational solution to an optimal control problem, allowing the controller designer to explore the tradeoff between architectural complexity and closed loop performance by varying the weight on the atomic norm penalty in the resulting convex optimization problem.  

In \cite{MC_RFD_TAC} we give explicit constructions of atomic norms useful for the design of actuation, sensing and joint actuation/sensing architectures, but do not address how to construct an atomic norm for communication architecture design.  Indeed constructing a suitable atomic norm for communication architecture design has substantial technical challenges that do not arise in actuation and sensing architecture design: we address these challenges in this paper.
We model a distributed controller as a collection of sub-controllers, each equipped with a set of actuators and sensors, that exchange their respective measurements with each other subject to \emph{communication delays} imposed by an underlying communication graph.  Keeping with the philosophy adopted in RFD \cite{MC_RFD_TAC}, we view dense communication architectures, i.e., ones with a large number of communication links between sub-controllers, as being composed of multiple simple \emph{atomic} communication architectures, i.e., ones with a small number of communication links between sub-controllers. 
% Although in general controllers with dense communication schemes will outperform controllers with sparser ones, it is desirable to minimize the cost of building the communication architecture needed to implement the controller.  
Thus the problem of controller communication architecture/control law co-design can be framed as the joint optimization of a suitably defined measure of the communication complexity of the distributed controller and its closed loop performance, in which these two competing metrics are traded off against each other in a principled manner.

The question that then needs to be answered is what properties should the designed communication architecture satisfy.  In general one can select communication architectures that range in complexity from completely decentralized, i.e., distributed controllers with no communication allowed between sub-controllers, to essentially centralized and without delay, i.e., distributed controllers with instantaneous communication allowed between all sub-controllers.  However, if we demand that the distributed optimal controller restricted to the designed communication architecture be specified in terms of the solution to a convex optimization problem then this limits the simplicity of the designed communication scheme \cite{W68,RL06,RCL10,LL11_QI}.  In particular a sufficient, and under mild assumptions necessary, condition for a distributed optimal controller to be specified by the solution to a convex optimization problem\footnote{For a more detailed overview of the relationship between information exchange constraints and the convexity of distributed optimal control problems, we refer the reader to \cite{RL06,RCL10,MMRY12} and the references therein.}  is that the communication architecture allow sub-controllers to communicate with each other as quickly as their control actions propagate through the plant \cite{RCL10}.  Although this condition may seem restrictive, it can often be met in practice by constructing a communication topology that mimics or is a superset of the physical topology of the plant.  For example, these delay based conditions could be satisfied in a smart-grid setting by laying down fiber-optic cables in parallel to transmission lines; in a SDN setting by giving control packets priority in routing protocols; and in an automated highway system setting by allowing vehicles to communicate wirelessly with nearby vehicles.

%Since this paper is about communication architecture design, I can ask the question of what type of architecture do we want to design and why?  I?d want something QI because it leads to convex optimal control problems, and I?d want something strongly connected because it makes these convex problems finite dimensional.  A simple condition for QI to hold is that the comms match the plant, something that can be generally accomplished in practice, e.g. in the power grid we would lay fiber optic cables along the power lines, in SDN we would give priority to control packets and in automated highway systems comms is wireless by the dynamics are decoupled.


%A useful approach to modeling a distributed plant is to view it as a collection of subplants that interact with each other according to \emph{propagation delays} imposed by their physical interconnection.  Likewise, a distributed controller can be viewed as a collection of sub-controllers, each equipped with a set of actuators and sensors, that exchange their respective measurements with each other subject to \emph{communication delays} imposed by an underlying communication graph.  
%With this view of distributed systems and distributed controllers, the communication architecture/control law co-design task is then to find a minimal set of communication links between sub-controllers such that a desired closed loop performance is achieved.  
%We additionally impose that the distributed optimal controller restricted to the designed communication architecture be linear and be specified by the solution to a convex optimization problem.  When these conditions on hold, it is then possible to determine the optimal performance achievable by a distributed controller implemented using the designed communication architecture, along with the optimal control law itself, allowing for a meaningful assessment of the quality of said architecture.

When the aforementioned delay based condition is satisfied by a distributed constraint, it is said to 
% In \cite{RL06}, the broadest known characterization of such convex distributed optimal control problems was made in terms of 
be \emph{quadratically invariant} (QI) \cite{RL06,RCL10}.  Although quadratic invariance guarantees convexity of the resulting distributed optimal control problem, it may still be infinite dimensional.  Recently it has been shown that in the case of $\Htwo$ distributed optimal control subject to QI constraints imposed by a strongly connected communication architecture, i.e. one in which every sub-controller can exchange information with every other sub-controller subject to delay, the resulting distributed optimal controller synthesis problem can be reduced to a finite dimensional convex program, and hence admits an efficient solution \cite{LDXX,LD14}.\footnote{Other solutions exist to the $\Htwo$ distributed control problem subject to delay constraints -- we refer the reader to the discussion and references in \cite{LD14} for a more extensive overview of this literature.}  In light of these observations, we therefore look to design \emph{strongly connected communication architectures} that induce \emph{QI} constraint sets -- once such a communication architecture is obtained, the methods from \cite{LDXX,LD14} can then be used to compute the optimal distributed controller restricted to that communication architecture exactly.

%
%
%Although we build on the methods presented in \cite{LDXX,LD14} to solve the $\Htwo$ distributed control problem subject to delays (which we review in \S \ref{sec:H2mm}),  we note that alternative solutions exist to this and other closely related controller synthesis problems, and refer the reader to \cite{LD14} for an extensive review of this literature.
%
%
%To solve the communication architecture/control law co-design problem, we observe that specific sparsity patterns in the impulse response elements of the controller have a direct interpretation in terms of the communication graph used by the controller, and hence we seek suitably structured solutions to the underlying distributed optimal controller synthesis problem.
To that end, we show that the communication complexity of a distributed controller can be inferred from the structure of its impulse response elements, allowing us to formulate the communication architecture/control law co-design task as one of seeking suitably structured solutions to an underlying controller synthesis problem.  
Inducing suitable structure in the solution to an optimization problem is of interest in a broad range of applications in applied mathematics, e.g., computing sparse solutions to linear inverse problems or computing low-rank solutions to systems of linear matrix equations is a problem that arises in signal processing and in statistics \ellcitations, \nuccitations. These ideas were extended in \cite{CRPW12}, where the authors describe a generic convex programming approach -- based on minimizing an appropriate \emph{atomic norm} \approxcitations$\text{ }$  -- for inducing a desired type of structure in solutions to linear inverse problems.  These techniques for inducing structure in the solution to a linear inverse problem were then suitably modified and applied to controller architecture design in \cite{MC_RFD_TAC} as part of the RFD framework.
%Motivated by these developments, our approach to the problem of joint communication architecture/control law co-design is to augment the variational formulation of the solution to the $\Htwo$ distributed optimal controller synthesis problem presented in \cite{LD14} with a suitable convex regularization function.% such that the structure of the solution to the regularized optimization problem corresponds to a strongly connected communication graph that induces a quadratically invariant constraint set.

%
%By carefully constructing this regularization function, we  ensure that  
%
%Our objective in this paper is to formulate this joint optimization in the context of $\Htwo$ distributed optimal control as a finite dimensional convex optimization problem.  We also ask that the optimal controller restricted to the designed communication architecture be linear and specified by the solution to a convex optimization problem that can be solved exactly.  In \cite{LDXX,LD14}, it is shown that if a strongly connected communication graph induces a \emph{quadratically invariant} \cite{RL06,RCL10} constraint set with respect to the distributed plant, then solving for the corresponding $\Htwo$ distributed optimal controller can be reduced to solving a finite dimensional convex quadratic program subject to affine constraints.  Further, it is seen that these affine constraints encode the communication architecture of the distributed controller.  Building on the results in \cite{LDXX,LD14}, our approach is to remove the affine constraints that encode the communication architecture of the distributed controller from the convex optimization problem, and instead augment the objective of this optimization problem with the a term that penalizes the communication complexity of the controller.




%Our approach is to augment the $\Htwo$ distributed optimal control problem with a suitable penalty such that the solution to the optimization problem specifies a communication architecture that is strongly connected and that induces induce a \emph{quadratically invariant} \cite{RL06,RCL10} constraint set with respect to the given distributed system.  These two properties of the designed communication architecture, namely quadratic invariance and strong connectedness, allow us to leverage the results of \cite{LDXX,LD14} 
%
%The quadratically invariant property of the constraint set ensures that the optimal controller restricted to the designed communication architecture is linear and specified as the solution of a convex optimization problem \cite{RL06,RCL10}.  The strong connectedness of the communication architecture allows us to leverage the recent results in \cite{LDXX,LD14} that reduce the controller synthesis problem to a finite dimensional convex quadratic program.


%The set of possible communication topologies between sub-controllers is combinatorial in cardinality, ranging from completely decentralized (i.e., no communication between sub-controllers) on one extreme to completely centralized (i.e., instantaneous communication between all sub-controllers) on the other.  However it is often the case that instantaneous communication between all sub-controllers is not possible due to finite communication speed and potentially physically dispersed systems.  On the other hand, it is well known that completely decentralized

\textbf{Related Work:}  Regularization techniques based on atomic norms have already been employed to great success in system identification \cite{SBTR12,Fazel,MR_CDC14,LjungNewOld}.
%Although the resulting solutions yield structured systems, they typically do not have a direct interpretation in terms of the architecture of a control system (i.e., actuators, sensors and the communication links between them).  
The use of regularization explicitly for the purpose of designing the architecture of a controller can also be found in the literature beyond the methods presented in \cite{MC_RFD_TAC}.  Representative examples include the use of $\ell_1$ regularization to design sparse structures in $\mathcal{H}_2$ feedback gains \cite{LFJ13}, treatment therapies \cite{JRM14}, consensus \cite{DLFM12,XB07} and synchronization \cite{FLJ13} topologies; and the use of group norm penalties to design actuation/sensing schemes \cite{MC_CDC14,DJL14}. 

\textbf{Contributions:}
%We formulate the communication architecture/control law co-design task as one of jointly optimizing the closed loop performance of a distributed controller and the complexity of the communication graph used to implement it, and show that this task can be accomplished via convex programming.  In particular 
% main contribution is the atomic norm
Our main contribution is an explicit construction of an atomic norm \cite{CRPW12}, \approxcitations, which we call the communication link norm, that can be incorporated into the RFD framework \cite{MC_RFD_TAC} to design strongly connected communication graphs that generate QI subspaces.  As argued above, these two structural properties allow for the distributed optimal controller implemented using the designed communication architecture to be specified by the solution to a finite dimensional convex optimization problem \cite{LDXX,LD14}.  We also show that by augmenting the variational solution to the $\Htwo$ distributed optimal control problem presented in \cite{LDXX,LD14} with the communication link norm as a regularizer, the communication architecture/control law co-design problem can be formulated as a second order cone program.  By varying the weight on the communication link norm penalty function, the controller designer can use our co-design algorithm to explore the tradeoff between communication architecture complexity and closed loop performance in a principled way via convex optimization. We use these results to formulate a communication architecture/control law co-design algorithm that yields a distributed optimal controller and the communication architecture on which it is to be implemented. 
%
%We show that adding a carefully constructed atomic norm as a convex penalty function to the variational solution to an optimal control problem induces structure in the resulting controller that specifies a strongly connected communication graph that leads to QI constraints.  These two structural properties of the designed communication graph allow us to leverage the results 
%
% intuitively, this norm penalizes the number of additional communication links used by the resulting distributed optimal controller.  We show that augmenting the variational solution to the $\Htwo$ distributed control problem presented in \cite{LDXX,LD14} with the communication link norm as a regularizer induces suitable structure in the solution of the resulting optimization problem.    
%In particular, the structure of this solution can be used to specify a strongly connected communication graph that leads to QI constraints,
%%that is both strongly connected and that leads to quadratically invariant constraints on the distributed controller.  These two properties allow for
%allowing for the resulting distributed optimal controller to be specified by the solution to a finite dimensional quadratic program \cite{LD14}. We use these results to formulate a communication architecture/control law co-design algorithm that yields a distributed optimal controller and the communication architecture on which it is to be implemented. By varying the weight on the communication link norm penalty function, the controller designer can use our co-design algorithm to explore the tradeoff between communication architecture complexity and closed loop performance in a principled way via convex optimization.  %We also note that the proposed communication link norm can be used in the RFD framework \cite{MC_RFD_TAC} to address the problem of joint actuation, sensing and communication architecture co-design.

\textbf{Paper Organization:}
In \S \ref{sec:prelims} we introduce necessary operator theoretic concepts and establish notation.   In \S \ref{sec:problem} we formulate the communication architecture/control law co-design problem as the joint optimization of a suitably defined measure of the communication complexity of a distributed controller and the closed loop performance that this controller achieves.  In \S \ref{sec:delays}, we show how communication graphs can be used to generate distributed constraints, and show that if a communication graph that generates a QI subspace is augmented with additional communication links, the subspace generated by the resulting communication graph is also QI.  We use this observation and techniques from structured linear inverse problems \cite{CRPW12} in \S \ref{sec:co_design} to construct a convex penalty function that penalizes the use of additional communication links by a distributed controller, and formulate the co-design procedure.  We discuss the computational complexity of the co-design procedure in \S \ref{sec:examples} and illustrate the usefulness of our approach with two numerical examples.  We end with a discussion in \S \ref{sec:discussion}.
